Permute-and-Flip: A new mechanism for differentially private selection

We consider the problem of differentially private selection. Given a finite set of candidate items and a quality score for each item, our goal is to design a differentially private mechanism that returns an item with a score that is as high as possible. The most commonly used mechanism for this task is the exponential mechanism. In this work, we propose a new mechanism for this task based on a careful analysis of the privacy constraints. The expected score of our mechanism is always at least as large as the exponential mechanism, and can offer improvements up to a factor of two. Our mechanism is simple to implement and runs in linear time.

==> concave.tex <==
\section{Maximizing Concave functions}

We now discuss how our mechanism can be applied when $n=\infty$, and our quality function is concave with respect to the output of the mechanism.  This setting will typically arise in settings where we are trying to learn some model parameters for the purposes of classification.  There, the desired output of the mechanism is model parameters $\theta$, which we want to choose to maximize some concave function $q(\theta, D)$ such as the log-likelihood.  Using notation consistent with the rest of this document, we can write $q_\theta$ to denote the quality of parameters $\theta$.  

The main idea to apply our mechanism to the case where $n=\infty$ is to first identify $q_*$ by solving the concave optimization problem, then repeatedly sample $\theta$ from some arbitrary distribution (that doesn't depend on the data), and flip the biased coin, returning $\theta$ if the coin comes up heads.  If $\theta$ is sampled from a uniform distribution, then this is the direct analogue of our mechanism (or the exponential mechanism), and using different sampling distributions biases the output towards certain $\theta$. 

Unforuntunately, running the mechanism as described above will literally take forever in general, unless the sampling distribution happens to sample near-optimal points with non-trivial probability.  However, we can still efficiently sample from the implied distribution using rejection sampling.  To do so, let's first investigate the density function:

$$ f(\theta) \propto \exp{\Big(\frac{\epsilon}{2} (q_{\theta} - q_*)\Big)} \propto \exp{\Big(\frac{\epsilon}{2} q_{\theta}\Big)} $$

Because $q_{\theta}$ is a concave function, $f$ is a \emph{log-concave} density.  This is important, because we know how to \emph{exactly} and efficiently sample from log-concave densities using rejection sampling. 

Therefore, as long as $q$ is a concave function (w.r.t $\theta$) and has bounded sensitivity (w.r.t. $D$), we can run the exponential mechanism when $n=\infty$ to solve the optimization problem under differential privacy. 

A natural follow-up question is whether we expect $q$ to satisfy these assumptions in general.  Consider one example: the log-likelihood for logistic regression:

$$ q_{\theta} = \sum_{i=1}^n \log{(1 + \exp{(-y_i \theta^T x_i)})} $$ 

While this function is concave, it has unbounded sensitivity in general.  This is because we can introduce a datapoint that makes a model predict it is $1$ with near certainty, but actually make it $-1$, which will blow up the objective.  Note that even if we add a regularization term, this does not affect the sensitivity of the function.  To bound the impact of any single individual, we could instead consider the related objective functions:

$$ q_{\theta} = \sum_{i=1}^n \min{\{\alpha, \log{(1 + \exp{(-y_i \theta^T x_i)})}\}} $$ 

$$ q_{\theta} = \sum_{i=1}^n \Big(y_i - \frac{1}{1 + \exp{(-\theta^T x_i)}} \Big)^2 $$  

These functions are both low-sensitivity approximations of our original objective, that limit the impact outliers can have.  Unfortunately, neither of them are concave.  Hence, it is not clear whether there exists an application for this nice idea.  


==> derivation.tex <==
\section{Derivation}

In this section we give the principles underlying our mechanism and the intuitions of the derivation.  
In this section, we show how our mechanism stated in Algorithm ? was derived.  The derivation is enlightening, as it directly shows how our mechanism addresses a longstanding suboptimality of the exponential mechanism.

\begin{obs}[Suboptimality of the Exponential Mechanism] \label{obs:suboptimality}
The Exponential Mechanism does not tightly satisfy the constraints required for differential privacy.  For $\q = (0,0)$ and $ \epsilon = 1$,
$$ \log{ \Big( \max_{q' \sim q} \frac{p_r(q)}{p_r(q')} \Big) } \approx 0.620115 < 1$$
\end{obs} 

This observation is problematic for the exponential mechanism, because it demonstrates that it is in some sense ``wasting'' the privacy budget.  A natural question follows from this observation: is the problem with the analysis of the exponential mechanism, or the mechanism itself?  While the ratio is not tight for this particular quality score, it gets arbitrarily close to $\epsilon$ for other quality scores (e.g., $ \q = (-10\Delta, 0)$).  Hence, the worst-case ratio between any pair of neighboring quality score vectors still approaches $\epsilon$, so the analysis of the exponential mechanism cannot be improved in general.

Instead, we derive a new mechanism for which these privacy constraints are tight \emph{by construction} for all quality score vectors.  First we establish some desiderata for our mechanism:

For now assume $q_* = 0$ and $q_i$ is an even integer for all $q_i$.  We will construct our mechanism one probability at a time, starting with the base case $ \q = \vec{0}$.  Clearly, by the symmetry requirement, we need $p_r(\vec{0}) = \frac{1}{n} $ for all $r$.   We want $p_*(\q)$ to be as large as possible, or equivalently $p_i(\q) $ to be as small as possible whenever $q_i < q_*$.  By the privacy, monotonicity, and regularity of our mechanism, $p_i$ must be at least as large as:

\begin{align*} 
p_r(q_1, \dots, q_r, \dots, q_n) &\geq \exp{(-\epsilon)} p_r(q_1 \pm 1, \dots, q_r \pm 1, \dots, q_n \pm 1) \\
&\geq \exp{(-\epsilon)} p_r(q_1 - 1, \dots, q_r + 1, \dots, q_n - 1) \\
&= \exp{(-\epsilon)} p_r(q_1, \dots, q_r + 2, \dots, q_n)
\end{align*}

We want this constraint to be tight, so we can treat this inequality as an equality.  This equation is a recursive definition for $p_r(\q)$, as it's value depends on the value of $p_r(\q')$ for some other $\q'$.  Note that this 



==> pareto_proof.tex <==

\pareto*
\begin{proof}
Note that the expected error of the mechanism can be expressed as:
%
\begin{align*}
\F(\M, \q) % &=\sum_{r \in \R} \Pr[\M(\q) = r] (q_* - q_r) \\
&= \sum_{\substack{r \in \R \\ q_r < q_*}} \Pr[\M(\q) = r] (q_* - q_r)
\end{align*}
Since $\F(\PF, \q) > \F(\M, \q)$, then $\Pr[\PF(\q) = r] > \Pr[\M(\q) = r]$ for some $r$ where $ q_r < q_* $.  By \cref{lem:pareto}, there must be some $\qq$ where $\F(\M, \qq) > \F(\PF, \qq)$.  This completes the proof.
\end{proof}


\begin{lemma} \label{lem:pareto}
If $\Pr[\M(\q) = r] < \Pr[\PF(\q) = r]$ for some $r$ where $q_r < q_*$, then there exists a $\qq$ such that $\F(\M, \qq) > \F(\PF, \qq)$.  
\end{lemma}

\begin{proof}
Let $\pvec{q}' = \q + (q_* - q_r) \e_r$.  
By the differential privacy and regularity of $\M$ and the recursive construction of $\PF$, we know:

\begin{align*}
\Pr[\M(\q) = r] &\geq \exp{\Big(\frac{\epsilon}{2 \Delta} (q_r - q_*)\Big)} \Pr[\M(\pvec{q}') = r] \\
\Pr[\PF(\q) = r] &= \exp{\Big(\frac{\epsilon}{2 \Delta} (q_r - q_*)\Big)} \Pr[\PF(\pvec{q}') = r] \\
\end{align*}
%
Combining the above with the assumption of the Lemma, we obtain:
%
$$ \Pr[\M(\pvec{q}) = r] < \Pr[\PF(\pvec{q}) = r] $$
%
Note that $\qq_r = \qq_*$.  We proceed by way of induction:

\textbf{Base Case:} $n'_* = n-1$.

There is a single $s$ such that $q'_s < q'_*$, and it must be the case that $\Pr[\M(\qq) = s] > \Pr[\PF(\qq) = s]$ by the symmetry and sum-to-one constraint on $\M$ and $\PF$.  Thus, it follows immediately that $ \F(\PF,\qq) < \F(\M,\qq)$ because $\M$ places more probability mass on the candidate $s$ that increases the expected error (i.e., $q'_* - q'_s > 0$). 

\textbf{Induction Step:} Assume \cref{lem:pareto} holds when $n'_* = k+1$.  We will show that \cref{lem:pareto} holds for $n'_* = k$.

We proceed in two cases:

\textbf{Case 1:} $ \Pr[\M(\qq) = s] \geq \Pr[\PF(\qq) = s]$ for all $s$ such that $ q'_s < q'_*$.   

The inequality must be strict for some $s$, because the inequality is strict for all $r$ where $q_r = q_*$ by the regularity/symmetry of $\M$ and $\PF$.  Thus, it follows immediately that $ \F(\PF,\qq) < \F(\M,\qq)$ because $\M$ places more probability mass on the candidates $s$ that increase the expected error (i.e., $q'_* - q'_s > 0$). 

\textbf{Case 2:} $\Pr[\M(\qq) = s] < \Pr[\PF(\qq) = s]$ for some $s$ such that $ q'_s < q_*$.  

Applying the induction hypothesis \cref{lem:pareto} using $\qq$ (now with $n'_* = k + 1$), we see that the claim must be true for $n'_* = k$, as desired.

\end{proof}


==> proof_empf.tex <==
%\subsection{Proof of \cref{thm:empf}}

\empf*

\begin{proof}%[Proof of \cref{thm:empf}]
The proof follows directly from \cref{lemma:step1} and \cref{lemma:step2} using  
$f_r = \Pr[\PF(\q) = r] - \Pr[\EM(\q) = r] $.
\end{proof}

\begin{lemma} \label{lemma:step1}
If $\Pr[\PF(\q) = r] - \Pr[\EM(\q) = r] \leq 0 $ and $ \Pr[\PF(\q) = s] - \Pr[\EM(\q) = s] > 0$ then $ q_r \leq q_s $.
\end{lemma}

\begin{proof}
Observe that $\Pr[\PF(\q) = r] - \Pr[\EM(\q) = r]$ can be expressed as $ p_r [g_r(\q) - h_r(\q)] $, where

\begin{align*}
g_r(\q) &= \frac{1}{n!} \sum_{\pi} \prod_{t : \pi(t) < \pi(r)} (1 - p_t) \\
%g_i(\q) &= \sum_{\substack{J \subseteq [n] \\ i \notin J}} \frac{(-1)^{|J|}}{|J|+1} \prod_{j \in J} \exp{\Big(\frac{\epsilon}{2} (q_j-q_*) \Big)} \\
h_r(\q) &= \frac{1}{\sum_{t \in \R} p_t}
\end{align*}

Further, notice that $h_r$ is constant with respect to $r$, and from \cref{lemma:step1a}, we know that $g_r$ is monotonic (i.e., $q_r \leq q_s \rightarrow g_r \leq g_s$).  Since the common term $p_r$ is non-negative, if $ \Pr[\PF(\q) = r] - \Pr[\EM(\q) = r] \leq 0$ then it must be the case that $g_r(\q) - h_r(\q) \leq 0$.  Similarly, if $\Pr[\PF(\q) = s] - \Pr[\EM(\q) = s] > 0$, then $g_s(\q) - h_s(\q) > 0$. By the monotonicity of $g$ (and hence $g - h$), we know that $q_r \leq q_s$ as desired.
\end{proof}

\begin{lemma} \label{lemma:step1a}
If $q_r \leq q_s$, then $g_r(\q) \leq g_s(\q)$, where

$$ g_r(\q) = \frac{1}{n!} \sum_{\pi} \prod_{t : \pi(t) < \pi(r)} (1 - p_t) $$
\end{lemma}

\begin{proof}

Note that if $ q_r \leq q_s$ then $1 - p_r \geq 1 - p_s$.  We will show that $g_s(\q) - g_r(\q) \geq 0$.

\begin{align*}
g_s(\q) - g_r(\q) &= \frac{1}{n!} \sum_{\pi} \Big[\prod_{t : \pi(t) < \pi(s)} (1-p_t) - \prod_{t : \pi(t) < \pi(r)} (1-p_t) \Big] \\
&\stackrel{(a)}{=} \frac{1}{n!} \sum_{\pi : \pi(r) < \pi(s)} \Big[\prod_{t : \pi(t) < \pi(s)} (1-p_t) - \prod_{k : \pi(t) < \pi(r)} (1-p_t) \Big]  \\
&+ \frac{1}{n!} \sum_{\pi : \pi(r) > \pi(s)} \Big[\prod_{t : \pi(t) < \pi(s)} (1-p_t) - \prod_{t : \pi(t) < \pi(r)} (1-p_t) \Big] \\
&\stackrel{(b)}{=} \frac{1}{n!} \sum_{\pi : \pi(r) < \pi(s)} \prod_{t : \pi(t) < \pi(s)} (1-p_t)
- \frac{1}{n!} \sum_{\pi : \pi(r) > \pi(s)} \prod_{t : \pi(t) < \pi(r)} (1-p_t) \\
&\stackrel{(c)}{=} \frac{1}{n!} \sum_{\pi : \pi(r) < \pi(s)} (1-p_r) \prod_{\substack{t : \pi(t) < \pi(s) \\ t \neq r}} (1-p_t)
- \frac{1}{n!} \sum_{\pi : \pi(r) > \pi(s)} (1-p_s) \prod_{\substack{t : \pi(t) < \pi(r) \\ t \neq s}} (1-p_t) \\
&\stackrel{(d)}{=} (p_s - p_r) \Big[\frac{1}{n!} \sum_{\pi : \pi(r) < \pi(s)} \prod_{\substack{t : \pi(t) < \pi(s) \\ t \neq s}} (1-p_t) \Big]\\
&\stackrel{(e)}{\geq}  0
\end{align*}

Above, (a) breaks the sum up into permutations where $r$ precedes $s$ and vice versa. Step (b) cancels common terms (those that do not contain $1-p_r$ or $1-p_s$).  Step (c) makes the dependence on $1-p_r$ and $1-p_s$ explicit.  Step (d) rearranges terms and uses a variable replacement on the second sum (replacing $r$ with $s$).  Step (e) uses the fact that both terms are non-negative.  
\end{proof}


\begin{lemma} \label{lemma:step2}
Let $\q,\vec{f}$ be arbitrary vectors satisfying:
\begin{enumerate}
\item $f_i \leq 0, f_j > 0 \rightarrow q_i \leq q_j$ 
\item $\sum_{i=1}^n f_i = 0$
\end{enumerate}
Then the following holds:
$$\sum_{i=1}^n q_i f_i \geq 0 $$
\end{lemma}

\begin{proof}
Assume without loss of generality $f_1 \leq f_2 \leq \dots \leq f_n$, and let $m$ be the index satisfying $ f_m \leq 0 $ and $f_{m+1} > 0$.  Then we have:

\begin{align*}
\sum_{i=1}^n q_i f_i &= \sum_{i=1}^m q_i f_i + \sum_{i=m+1}^n q_i f_i \\
&\stackrel{(a)}{\geq} \big(\max_{1 \leq i \leq m} q_i\big) \sum_{i=1}^m f_i + \big(\min_{m < i \leq n} q_i\big) \sum_{i=m+1}^n f_i \\
&\stackrel{(b)}{=} [\min_{m < i \leq n} q_i - \max_{1 \leq i \leq m} q_i] \Big(\sum_{i=m+1}^n f_i \Big) \\
&\stackrel{(c)}{\geq} 0
\end{align*}
Above, (b) follows from the fact that $\sum_{i=1}^m f_i = -\sum_{i=m+1}^n f_i $ (by condition 2), and (c) follows from the fact that both terms in the product are non-negative (by condition 1).


\end{proof}




==> proofs_mechanism.tex <==
\section{Proofs} \label{sec:proofs}

We begin by deriving two expressions for the probability mass function.

%\pmf*
\begin{restatable}{theorem}{pmf} \label{thm:pmf}
Two expressions for the probability mass function of $\M_{PF}$ are:
\begin{align*}
Pr[\M_{PF}(\q) = r]
%&= \frac{1}{n!} \exp{\big(\frac{\epsilon}{2 \Delta} (q_i - q_*)\big)} \sum_{\pi} \prod_{j : \pi(j) < \pi(i)} \big[1 - \exp{\big(\frac{\epsilon}{2 \Delta} (q_j - q_*)\big)}\big] \\
%&= \exp{\big(\frac{\epsilon}{2 \Delta} (q_i - q_*)\big)} \sum_{\substack{J \subseteq [n] \\ i \notin J}} \frac{(-1)^{|J|}}{|J|+1} \prod_{j \in J} \exp{\big(\frac{\epsilon}{2 \Delta} (q_j - q_*)\big)} \\
&= p_r \sum_{\pi} \frac{1}{n!} \prod_{s : \pi(s) < \pi(r)} (1 - p_s) \\
&= p_r \sum_{\substack{S \subseteq \R \\ r \notin S}} \frac{(-1)^{|S|}}{|S|+1} \prod_{s \in S} p_s \\
\end{align*} 
where $\pi$ is a permutation and $p_r = \exp{\big( \frac{\epsilon}{2 \Delta} (q_r - q_*)\big)} $.  
\end{restatable}


\begin{proof}%[Proof of \cref{thm:pmf}]

Let $X_r \sim Bernoulli(p_r)$ denote the random coin flip for item $r$ and let $\pi$ be a random permutation.

\textbf{Expression 1:}
\begin{align*}
\Pr[\PF(\q) = r] &= Pr[X_r \wedge_{s : \pi(s) < \pi(r)} \neg X_s] \\
&= \frac{Pr[X_r]}{n!} \sum_{\pi} \prod_{s : \pi(s) < \pi(r)} (1 - Pr[X_s]) \\
&= \frac{p_r}{n!} \sum_{\pi} \prod_{s : \pi(s) < \pi(r)} (1 - p_s) \\
\end{align*}

\textbf{Expression 2:}

Alternatively, using the inclusion exclusion principle:

\begin{align*}
\Pr[\PF(\q) = r] &= Pr[X_r \wedge \neg \vee_{s \neq r} [X_s \wedge \pi(s) < \pi(r)]] \\
&= Pr[X_r] (1 - Pr[\vee_{s \neq r} [X_s \wedge \pi(s) < \pi(r)]]) \\
&= Pr[X_r] \Big[1 - \sum_{\substack{S \subseteq \R \\ r \notin S \\ |S| \geq 1}} (-1)^{|S|} Pr[\wedge_{s \in S} [X_s \wedge \pi(s) < \pi(r)]]\Big] \\
&= Pr[X_r] \Big[1 - \sum_{\substack{S \subseteq \R \\ r \notin S \\ |S| \geq 1}} (-1)^{|S|} Pr[\wedge_{s \in S} \pi(s) < \pi(r)] Pr[\wedge_{s \in S} X_s] \Big] \\
&= Pr[X_r] \Big[1 - \sum_{\substack{S \subseteq \R \\ r \notin S \\ |S| \geq 1}} (-1)^{|S|} \frac{1}{|S|+1} \prod_{s \in S} Pr[X_s] \Big] \\
&= Pr[X_r] \sum_{\substack{S \subseteq \R \\ r \notin S}} \frac{(-1)^{|S|}}{|S|+1} \prod_{s \in S} Pr[X_s] \\
&= p_r \sum_{\substack{S \subseteq \R \\ r \notin S}} \frac{(-1)^{|S|}}{|S|+1} \prod_{s \in S} p_s \\
\end{align*}

\end{proof}

\regdp*
\begin{proof}%[Proof of \cref{prop:regdp}]

Let $\M$ be a regular mechanism satisfying:
\begin{equation} \label{eq:regdpassumption}
\Pr[\M(\q) = r] \geq \exp{(-\epsilon)} \Pr[\M(\q + 2\Delta\e_r) = r] 
\end{equation}

Our goal is to show that $\M$ is differentially private, i.e., if for all $\q \in \mathbb{R}^{\R}$, $r\in\R$, and $\vec{z} \in [-\Delta, \Delta]^{\R}$,
$$ \Pr[\M(\q) = r] \leq \exp{(\epsilon)} \Pr[\M(\q + \vec{z}) = r] $$

Using this assumption together with the regularity of $\M$, we obtain:

\begin{align*}
\Pr[\M(\q) = r] &\leq \exp{(\epsilon)} \Pr[\M(\q - 2\Delta\e_r) = r] && \text{by \cref{eq:regdpassumption}} \\
&= \exp{(\epsilon)} \Pr[\M(\q + \Delta \vec{1} - 2\Delta\e_r) = r]  && \text{by shift-invariance} \\
&\leq \exp{(\epsilon)} \Pr[\M(\q + \vec{z}) = r] && \text{by monotonicity} \\
\end{align*}
Thus, we conclude that $\M$ is differentially-private, as desired.  This completes the proof.
\end{proof}





\pfdp*
\begin{proof}%[Proof of \cref{thm:dp}]
We first argue that $\PF$ is regular.   %Below we show that it is symmetric.

%\begin{align*}
%\Pr[\PF(\Pi \q) = \pi(r)] &= (\Pi p)_{\pi(r)} \sum_{\sigma} \frac{1}{n!} \prod_{s : \sigma(\pi(s)) < \sigma(\pi(r))} (1 - (\Pi p)_{\pi(s)}) \\
%&= p_r \sum_{\sigma} \frac{1}{n!} \prod_{s : \sigma(\pi(s)) < \sigma(\pi(r))} (1 - p_s) \\
%&= p_r \sum_{\sigma} \frac{1}{n!} \prod_{s : \sigma(s) < \sigma(s)} (1 - p_s) \\
%&= \Pr[\PF(\q) = r] 
%\end{align*}
%\ry{seems like overkill for something trivial}

\textbf{Symmetry}:
Consider $p_r$ as defined in the definition of $\PF$, and let $\pvec{p}' = \Pi \vec{p}$ denote the same vector on the permuted quality scores.  Now note that every permutation is equally likely for both $\vec{p}$ and $\pvec{p}'$, and that the only difference is that $p_r = p'_{\pi(r)}$.  Hence $\Pr[\M(\q) = r] = \Pr[\M(\Pi \q) = \pi(r)]$, which implies $\M$ is symmetric as desired.

\textbf{Shift-invariance}:
The mechanism is shift-invariant because on only depends on $\q$ through $ q_r - q_*$.  Specifically, we have $p_r = \exp{(\frac{\epsilon}{2 \Delta} (q_r - q_*))} = \exp{\big(\frac{\epsilon}{2 \Delta} ((q_r + c) - (q_* + c))\big)}$, and hence $\Pr[\M(\q) = r] = \Pr[\M(\q + c \vec{1}) = r] $ as desired.

\textbf{Monotonicity}:
Monotonicity follows immediately from the pmf of the mechanism.  

$$ \Pr[\PF(\q) = r] = p_r \sum_{\pi} \frac{1}{n!} \prod_{s : \pi(s) < \pi(s)} (1 - p_s) $$

Assume without loss of generality that $q_* = 0$ and note that $p_r = \exp{(\frac{\epsilon}{2 \Delta} q_r)}$.  Clearly, the expression above is monotonically increasing in $p_r$ (and hence $q_r$) and monotonically decreasing in $p_s$ (and hence $q_s$).  Hence $\PF$ satisfies the monotonicity property.

Because $\PF$ is symmetric, shift-invariant, and monotonic, it is regular.

We now argue that $\PF$ is differentially-private.  By \cref{prop:regdp}, it suffices to show that 
$$ \Pr[\M(\q) = r] \geq \exp{(-\epsilon)} \Pr[\M(\q + 2 \Delta e_r) = r]$$
or equivalently,

$$ \log \Pr[\M(\q) = r] \leq \epsilon + \log \Pr[\M(\q - 2 \Delta e_r) = r] $$

Let $ f_r(\q) = \log \Pr[\M(\q) = r] $ and note that it is enough to show that $\frac{\partial f_r}{\partial q_r} \leq \frac{\epsilon}{2 \Delta} $ for all $(\q, r)$.  

\textbf{Case 1:} $q_r < q_*$

\begin{align*}
\frac{\partial f_r}{\partial q_r} &= \frac{\partial f_r}{\partial p_r} \frac{\partial p_r}{\partial q_r} \\
&= \Big[ \frac{1}{\Pr[\M(\q) = r]} \sum_{\pi} \frac{1}{n!} \prod_{s : \pi(s) < \pi(r)} (1 - p_s) \Big] \Big[ p_r \frac{\epsilon}{2 \Delta} \Big] \\
&= \frac{\epsilon}{2 \Delta} \frac{\Pr[\M(\q) = r]}{\Pr[\M(\q) = r]} 
= \frac{\epsilon}{2\Delta} 
\end{align*}

\textbf{Case 2:} $q_r = q_*$

\begin{align*}
\frac{\partial f_r}{\partial q_r} &= \sum_{t} \frac{\partial f_r}{\partial p_t} \frac{\partial p_t}{\partial q_r} \\
&= \sum_{t \neq r} \Big[ -\frac{1}{\Pr[\M(\q) = r]} p_r \sum_{\pi : \pi(t) < \pi(r)} \frac{1}{n!} \prod_{\substack{s : \pi(s) < \pi(r) \\ s \neq t}} (1 - p_s) \Big] \Big[ -\frac{\epsilon}{2 \Delta} p_r \Big] \\
&= \frac{1}{\Pr[\M(\q) = r]} \Big[\sum_{t \neq r} p_r \sum_{\pi : \pi(t) < \pi(r)} \frac{1}{n!} \prod_{\substack{s : \pi(s) < \pi(r) \\ s \neq t}} (1 - p_s) \Big] \Big[ \frac{\epsilon}{2 \Delta} \Big] \\
&= \frac{1}{\Pr[\M(\q) = r]} \Big[\sum_{t \neq r} p_r \sum_{\pi : \pi(t) > \pi(r)} \frac{1}{n!} \prod_{\substack{s : \pi(s) < \pi(r)}} (1 - p_s) \Big] \Big[ \frac{\epsilon}{2 \Delta} \Big] \\
&= \Big[\sum_{t \neq r} \sum_{\pi : \pi(t) > \pi(r)} \frac{2 - p_t}{n!} \prod_{\substack{s : \pi(s) < \pi(r)}} (1 - p_s) \Big]^{-1}
\Big[\sum_{t \neq r} \sum_{\pi : \pi(t) > \pi(r)} \frac{1}{n!} \prod_{\substack{s : \pi(s) < \pi(r)}} (1 - p_s) \Big] \Big[ \frac{\epsilon}{2 \Delta} \Big] \\
&\leq \frac{\epsilon}{2 \Delta} 
%&\leq \frac{\epsilon}{2} \\
\end{align*}

Above, step (a) uses the chain rule.  Step (b) calculates the individual derivatives.  Step (c) cancels the negative terms and substitutes $p_r = 1$.  Step (d) uses the observation that the same sum can be expressed over a different set of permutations.  Step (e) writes $\Pr[\M(\q) = r]$ in a way that makes a direct comparison possible.  Step (f) uses the fact that the first term (denominator) is larger than the second term (numerator) (it attains equality when $p_t = 1$ for all $t$).

This completes the proof.

\end{proof}

\solution*
\begin{proof}%[Proof of \cref{prop:solution}]

%We will show that the Permute and Flip mechanism solves the recurrence relation. 

\textbf{Case 1:} $q_r = q_*$

Because $\PF(\q)$ is a valid probability distribution for all $\q$, and it is symmetric, it must satisfy case $2$ of the recurrence relation.


\textbf{Case 2:} $ q_r < q_* $ 

Note that the pmf of $\PF$ is:
\begin{align*}
\Pr[\M_{PF}(\q) = r] &= p_r \sum_{\pi} \frac{1}{n!} \prod_{s : \pi(s) < \pi(r)} (1 - p_s) \\
\Pr[\M_{PF}(\q + (q_* - q_r) \vec{e}_r) = r] &= p_r' \sum_{\pi} \frac{1}{n!} \prod_{s : \pi(s) < \pi(r)} (1 - p_s)
\end{align*}

where $p_r = \exp{(\frac{\epsilon}{2 \Delta} (q_r - q_*))}$ and $p'_r = \exp{(\frac{\epsilon}{2 \Delta} (q_* - q_*))} = 1$.  By comparing terms, it is clear that 
$$\Pr[\M_{PF}(\q) = r] = \exp{(\frac{\epsilon}{2 \Delta} (q_r - q_*))} \Pr[\M_{PF}(\q + (q_* - q_r) \vec{e}_r) = r] $$

Hence, $\PF$ solves case $1$ of the recurrence relation.  This completes the proof.

\end{proof}





==> symmetric.tex <==
\begin{lemma} \label{lemma:symmetric}
If
\begin{enumerate}
\item $g(x)$ is a negative, strictly convex function
\item $h(x)$ is a positive, linear, and monotonically decreasing function
\item $f(x,y) = g(x) h(y) + g(y) h(x) $
\end{enumerate}
 then for any $a \neq b \in Dom(f)$, there is a $c \in [a,b]$ such that $f(c,c) < f(a,b)$.
\end{lemma}
\begin{proof}
Without loss of generality, assume $a < b$.  We proceed in cases:

\textbf{Case 1:} $g(a) \leq g(b)$ \\
Set $c=a$.
\begin{align*}
f(c,c) &= g(a) h(a) + g(a) h(a) \\
&< g(a) h(b) + g(a) h(a) \\
&\leq g(a) h(b) + g(b) h(a) \\
\end{align*}
The first inequality comes from the fact that $h(a) > h(b)$ and $g(a) < 0$.  The second inequality comes from the fact that $g(a) \leq g(b)$ (Case 1) and $h(a) > 0$.

\textbf{Case 2:} $g(a) > g(b)$ \\
Set $c = \frac{a+b}{2}$.

\begin{align*}
f(c,c) &= 2 g(\frac{a+b}{2}) h(\frac{a+b}{2}) \\
&= g(\frac{a+b}{2}) [h(a)+h(b)] \\
&< \frac{1}{2} [g(a) + g(b)] [h(a) + h(b)] \\
&= \frac{1}{2} [g(a) h(a) + g(a) h(b) + g(b) h(a) + g(b) h(b)] \\
&< \frac{1}{2} [2 g(a) h(b) + g(b) h(a) + g(b) h(b)] \\
&< g(a) h(b) + g(b) h(a) \\
\end{align*}
The first inequality follows from the strict convexity of $g$ and the positivity of $h$.  The second inequality comes from the fact that $h(a) > h(b)$ and $g(a) < 0$.  The third inequality comes from the fact that $g(a) > g(b)$ (Case 2) and $h(a) > 0$.

This completes the proof.
\end{proof}



==> theory.tex <==
\begin{proof}[Proof of \cref{thm:empf}]
The proof follows directly from \cref{lemma:step1} and \cref{lemma:step2} using  
$f_i = p_i^{RM}(\q) - p_i^{EM}(\q)$.
\end{proof}

\begin{lemma} \label{lemma:step1}
If $p_i^{RM}(\q) - p_i^{EM}(\q) \leq 0 $ and $ p_j^{RM}(\q) - p_j^{EM}(\q) > 0$ then $q_i \leq q_j$.
\end{lemma}

\begin{proof}
Observe that $p_i^{RM}(\q) - p_i^{EM}(\q)$ can be expressed as $\exp{\big(\frac{\epsilon}{2} q_i\big)} [g_i(\q) - h_i(\q)] $, where

\begin{align*}
g_i(\q) &= \frac{1}{n!} \sum_{\sigma} \prod_{k : \sigma(k) < \sigma(i)} [1 - \exp{(\frac{\epsilon}{2} (q_k - q_*))}] \\
%g_i(\q) &= \sum_{\substack{J \subseteq [n] \\ i \notin J}} \frac{(-1)^{|J|}}{|J|+1} \prod_{j \in J} \exp{\Big(\frac{\epsilon}{2} (q_j-q_*) \Big)} \\
h_i(\q) &= \frac{1}{\sum_{j=1}^n \exp{\Big(\frac{\epsilon}{2} q_j\Big)}}
\end{align*}

Further, notice that $h_i$ is constant with respect to $i$, and from \cref{lemma:step1a}, we know that $g_i$ is monotonic (i.e., $q_i \leq q_j \rightarrow g_i \leq g_j$).  Since the common term $\exp{(\frac{\epsilon}{2} q_i)}$ is non-negative, if $ p_i^{RM}(\q) - p_i^{EM}(\q) \leq 0$ then it must be the case that $g_i(\q) - h_i(\q) \leq 0$.  Similarly, if $p_j^{RM}(\q)-p_j^{EM}(\q) > 0$, then $g_j(\q) - h_j(\q) > 0$. By the monotonicity of $g$ (and hence $g - h$), we know that $q_i \leq q_j$ as desired.
\end{proof}

\begin{lemma} \label{lemma:step1a}
If $q_i \leq q_j$, then $g_i(\q) \leq g_j(\q)$, where

$$ g_i(\q) = \frac{1}{n!} \sum_{\sigma} \prod_{k : \sigma(k) < \sigma(i)} [1 - \exp{(\frac{\epsilon}{2} (q_k - q_*))}] $$
\end{lemma}

\begin{proof}

Let $c_i = 1 - \exp{(\frac{\epsilon}{2} (q_i - q_*))}$, and note that if $ q_i \leq q_j$ then $c_i \geq c_j$.  We will show that $g_j(\q) - g_i(\q) \geq 0$.

\begin{align*}
g_j(\q) - g_i(\q) &= \frac{1}{n!} \sum_{\sigma} \Big[\prod_{k : \sigma(k) < \sigma(j)} c_k - \prod_{k : \sigma(k) < \sigma(i)} c_k \Big] \\
&\stackrel{(a)}{=} \frac{1}{n!} \sum_{\sigma : \sigma(i) < \sigma(j)} \Big[\prod_{k : \sigma(k) < \sigma(j)} c_k - \prod_{k : \sigma(k) < \sigma(i)} c_k \Big]  \\
&+ \frac{1}{n!} \sum_{\sigma : \sigma(i) > \sigma(j)} \Big[\prod_{k : \sigma(k) < \sigma(j)} c_k - \prod_{k : \sigma(k) < \sigma(i)} c_k \Big] \\
&\stackrel{(b)}{=} \frac{1}{n!} \sum_{\sigma : \sigma(i) < \sigma(j)} \prod_{k : \sigma(k) < \sigma(j)} c_k 
- \frac{1}{n!} \sum_{\sigma : \sigma(i) > \sigma(j)} \prod_{k : \sigma(k) < \sigma(i)} c_k \\
&\stackrel{(c)}{=} \frac{1}{n!} \sum_{\sigma : \sigma(i) < \sigma(j)} c_i \prod_{\substack{k : \sigma(k) < \sigma(j) \\ k \neq i}} c_k 
- \frac{1}{n!} \sum_{\sigma : \sigma(i) > \sigma(j)} c_j \prod_{\substack{k : \sigma(k) < \sigma(i) \\ k \neq j}} c_k \\
&\stackrel{(d)}{=} (c_i - c_j) \Big[\frac{1}{n!} \sum_{\sigma : \sigma(i) < \sigma(j)} \prod_{\substack{k : \sigma(k) < \sigma(j) \\ k \neq i}} c_k \Big]\\
&\stackrel{(e)}{=} \geq 0
\end{align*}

Above, (a) breaks the sum up into permutations where $i$ precedes $j$ and vice versa. Step (b) cancels common terms (those that do not contain $c_i$ or $c_j$).  Step (c) makes the dependence on $c_i$ and $c_j$ explicit.  Step (d) rearranges terms and uses a variable replacement on the second sum (replacing $i$ with $j$).  Step (e) uses the fact that both terms are non-negative.  
\end{proof}


\begin{lemma} \label{lemma:step2}
Let $\q,\vec{f}$ be arbitrary vectors satisfying:
\begin{enumerate}
\item $f_i \leq 0, f_j > 0 \rightarrow q_i \leq q_j$ 
\item $\sum_{i=1}^n f_i = 0$
\end{enumerate}
Then the following holds:
$$\sum_{i=1}^n q_i f_i \geq 0 $$
\end{lemma}

\begin{proof}
Assume without loss of generality $f_1 \leq f_2 \leq \dots \leq f_n$, and let $m$ be the index satisfying $ f_m \leq 0 $ and $f_{m+1} > 0$.  Then we have:

\begin{align*}
\sum_{i=1}^n q_i f_i &= \sum_{i=1}^m q_i f_i + \sum_{i=m+1}^n q_i f_i \\
&\stackrel{(a)}{\geq} \big(\max_{1 \leq i \leq m} q_i\big) \sum_{i=1}^m f_i + \big(\min_{m < i \leq n} q_i\big) \sum_{i=m+1}^n f_i \\
&\stackrel{(b)}{=} [\min_{m < i \leq n} q_i - \max_{1 \leq i \leq m} q_i] \Big(\sum_{i=m+1}^n f_i \Big) \\
&\stackrel{(c)}{\geq} 0
\end{align*}
Above, (b) follows from the fact that $\sum_{i=1}^m f_i = -\sum_{i=m+1}^n f_i $ (by condition 2), and (c) follows from the fact that both terms in the product are non-negative (by condition 1).
\end{proof}



==> theory2.tex <==
\section{Theoretical Results 2}

\begin{theorem}
$q_* - \E_{i \sim \M_{EM}(\q)}[q_i]$ is maximized when $\q = (c, \dots, c, 0)$ for some $ c < 0$.
\end{theorem}

\begin{proof}
The expected score of the mechanism can be expressed as:

$$ \E[q_i] = \sum_i q_i \frac{\exp{(\epsh q_i)}}{\sum_j \exp{(\epsh q_j)}} $$

Without loss of generality, assume $q_n = q_* = 0$ and make the substitution $p_i = \exp{(\epsh q_i)}$.  This becomes:

$$ \E[q_i] = \frac{2}{\epsilon} \frac{1}{\sum_j p_j} \sum_i p_i \log{(p_i)}  $$

Our goal is to show this is minimized when $p_1 = \cdots = p_{n-1} $.  We procede by way of contradiction.  Assume WLOG $p_1 < p_2$.  We will argue that we can replace $p_1$ and $p_2$ with new values that decrease the objective.  First write the expected score as a function of $p_1$ and $p_2$, treating everything else as a constant.  

$$ f(p_1, p_2) = \frac{1}{p_1 + p_2 + a} \big[p_1 \log{(p_1)} + p_2 \log{(p_2)} + b \big] $$

We will show that $f(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}) < f(p_1, p_2)$.  

\begin{align*}
f\big(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}\big) &= \frac{1}{2 \frac{p_1+p_2}{2}+a} [2 \frac{(p_1+p_2)}{2} \log{(\frac{p_1+p_2}{2})}+b] \\
&= \frac{1}{p_1+p_2+a} [2 \frac{(p_1+p_2)}{2} \log{(\frac{p_1+p_2}{2})}+b] \\
&< \frac{1}{p_1+p_2+a} [p_1 \log{(p_1)} + p_2 \log{(p_2)} + b] \\
&= f(p_1, p_2) \\
\end{align*}
Above, the inequality follows from the strict convexity of $p \log{(p)}$.  Thus, $f(p_1,p_2)$ is not a minimum, which is a contradiction.  This completes the proof.
\end{proof}

\begin{theorem}
$q_* - \E_{i \sim \M_{RM}(\q)}[q_i]$ is maximized when $\q = (c, \dots, c, 0)$ for some $ c < 0$.
\end{theorem}

\begin{proof}
Without loss of generality, assume $q_n = q_* = 0$.  The expected score of the mechanism can be written as:

$$ \E_{i \sim \M_{RM}(\q)}[q_i] = \sum_{i=1}^n q_i \exp{(\frac{\epsilon}{2} q_i)} \sum_{\sigma} \frac{1}{n!} \prod_{j : \sigma(j) < \sigma(i)} [1 - \exp{(\frac{\epsilon}{2} q_j)}] $$

Now consider a change of variables where $p_i = \exp{(\frac{\epsilon}{2} q_i)}$, and note that $p_i \in (0,1]$ and $p_n=1$.  Now define the function of the free variables $\p = (p_1, \dots, p_{n-1}) $: \footnote{note that $p_n=1$ is still defined as a global constant}.  

$$ f(\p) = \frac{2}{\epsilon} \sum_{i=1}^n \log{(p_i)} p_i \sum_{\sigma} \frac{1}{n!} \prod_{j : \sigma(j) < \sigma(i)} [1 - p_j] $$

We wish to show that this is minimized when $p_1 = \dots = p_{n-1} = c$ for some $c \in (0,1)$.  We proceed by way of contradiction.  Assume that $\p \neq c \vec{1}$, then we will show that there exists an $\r$ such that $f(\r) < f(\q)$.   Without loss of generality, assume $p_1 < p_2$, and look at $f$ as a function of only $p_1$ and $p_2$, treating everything else as a global constant.  Then $f$ can be expressed as:

$$ f(p_1, p_2) = p_1 \log{(p_1)} [a (1-p_2) + b] + p_2 \log{(p_2)} [a (1 - p_1) + b] - c (1-p_1) - c (1-p_2) - d (1-p_1) (1-p_2) - e$$

where $a,b,c,d,e \geq 0$.
We proceed in cases, by showing that we can always find new values for $p_1$ and $p_2$ that reduces $f$

\textbf{Case 1:} $p_1 \log{(p_1)} < p_2 \log{(p_2)}$

Set $p_2 \leftarrow p_1$. 

The second term in the sum is (strictly) less by the assumption of case 1.  Every other term is strictly less because $p_1 < p_2$, which implies $(1-p_1) > (1-p_2)$ or equivalently $-(1-p_1) < -(1-p_2)$.

\textbf{Case 2:} $p_1 \log{(p_1)} \geq p_2 \log{(p_2)}$

Set $p_1 = p_2 \leftarrow \frac{p_1 + p_2}{2} $. 

Consider breaking up the sum into two pieces; i.e., $ f(p_1, p_2) = f_A(p_1, p_2) + f_B(p_1, p_2) $ where:

\begin{align*}
f_A(p_1, p_2) &= p_1 \log{(p_1)} [a (1-p_2) + b] + p_2 \log{(p_2)} [a (1 - p_1) + b] \\
f_B(p_1, p_2) &= - c (1-p_1) - c (1-p_2) - d (1-p_1) (1-p_2) - e
\end{align*}

We have:

\begin{align*}
f_A(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}) &= 2 \frac{p_1+p_2}{2} \log{(\frac{p_1+p_2}{2})} (a (1 - \frac{p_1+p_2}{2}) + b) \\
&= (p_1 + p_2) \log{(\frac{p_1+p_2}{2})} [ a (1-p_1) + b + a (1-p_2) + b] \\
&< \frac{1}{2} [p_1 \log{(p_1)} + p_2 \log{(p_2)}] [a (1-p_1) + b + a(1-p_2) + b] \\
&= \frac{1}{2} \Big[ p_1 \log{(p_1)} [a (1-p_1) + b] + p_1 \log{(p_1)} [a (1-p_2) + b] \\ 
&\quad + \:\: p_2 \log{(p_2)} [ a (1-p_1) + b] + p_2 \log{(p_2)} [a (1-p_2) + b] \Big] \\
&< p_1 \log{(p_1)} [a (1-p_2) + b] + p_2 \log{(p_2)} [a (1-p_1) + b] \\
&= f_A(p_1, p_2) \\
%&= g(\frac{p_1+p_2}{2}) [h_A(p_1) + h_A(p_2)] \\
%&< \frac{1}{2} [g(p_1) + g(p_2)] [h_A(p_1) + h_A(p_2)] \\
%&= \frac{1}{2} [g(p_1) h_A(p_1) + g(p_1) h_A(p_2) + g(p_2) h_A(p_1) + g(p_2) h_A(p_2)] \\
%&< g(p_1) h_A(p_2) + g(p_2) h_A(p_1) \\
%&= f_{1..2}(p_1, p_2)
\end{align*}

Above, the first step follows from linearity, and the second step follows from the convexity of $p \log{(p)}$ and non-negativeness of the linear term.  The fourth step uses the assumption that $g(p_1) > g(p_2)$ (Case 2), and the fact that $a(1-p_1) + b > a(1-p_2) + b$ and $\log{(p_2)} < 0$.    

\begin{align*}
f_B(\frac{p_1+p_2}{2}) &= -2c (1-\frac{p_1+p_2}{2}) -d (1 - \frac{p_1+p_2}{2})^2 - e \\
&= -c (1-p_1) - c(1-p_2) - d (1 - \frac{p_1+p_2}{2})^2 - e \\
&< -c (1-p_1) - c(1-p_2) - d (1-p_1) (1-p_2) - e \\
&= f_B(p_1, p_2) \\
%f_{3..n}(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}) &= 2 h_B(\frac{p_1+p_2}{2}) + h_C(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}) \\
%&= h_B(p_1) + h_B(p_2) + h_C(\frac{p_1+p_2}{2}, \frac{p_1+p_2}{2}) \\
%&< h_B(p_1) + h_B(p_2) + h_C(p_1, p_2) \\
%&= f_{3..n}(p_1, p_2) \\
\end{align*}
Above, the first step follows from linearity, and the second step follows from the fact that the area of a square is always larger than the area of a rectangle with the same perimeter.  

We have shown that $f_A$ and $f_B$ are both reduced, so $f$ as a whole is also reduced.  This completes the proof.
\end{proof}

\begin{corollary}[Optimality] The expected utiltiy of our mechanism is always at least:
$$ \mathbb{E}[q_i] \geq q_* - \frac{2}{\epsilon} \Big[\max_{0 < p < 1} \log{(p)} \frac{1 - (1 - p)^n}{n p} - \log{(p)}\Big] $$
\end{corollary}

\begin{proof}
Recall in the worst case quality score vector is $\q = (c, \dots, c, 0)$ for some $c < 0$.  Adding a cosntant to each of these quality scores, we may instaed assume $\q = (0,\dots,0,q_*)$.  The expected score of our mechanism is 

$$ q_* \cdot \exp{(\frac{\epsilon}{2} 0)} \cdot \sum_{J \subseteq [n-1]} \frac{(-1)^{|J|}}{|J|+1} \prod_{j \in J } \exp{(-\frac{\epsilon}{2} q_*)} $$

Making the substitution $p = \exp{(-\frac{\epsilon}{2} q_*)}$ (equivalently $ q_* = -\frac{2}{\epsilon} \log{(p)}$) we arrive at:

\begin{align*}
\E[q_i] &= -\frac{2}{\epsilon} \log{(p)} \sum_{J \subseteq [n-1]} \frac{(-1)^{|J|}}{|J|+1} \prod_{j \in J} p \\
&= -\frac{2}{\epsilon} \log{(p)} \sum_{k=0}^{n-1} {n-1 \choose k} \frac{(-1)^{k}}{k+1} p^k \\
&= -\frac{2}{\epsilon} \log{(p)} \frac{1 - (1-p)^n}{n p} \\
\end{align*}

And the difference between $q_*$ and $\E[q_i]$ is thus:

\begin{align*}
q_* - \E[q_i] &= -\frac{2}{\epsilon} \Big[ \log{(p)} - \log{(p)} \frac{1 - (1-p)^n}{p n} \Big] \\
&= \frac{2}{\epsilon} \Big[ \log{(p)} \frac{1 - (1-p)^n}{p n} - \log{(p)} \Big] \\
\end{align*}

Maximizing this difference over $p$ leads to the stated result.
\end{proof}

\begin{theorem}
$$ \max_{0 < p < 1} \log{(p)} \frac{1 - (1-p)^n}{n p} - \log{(p)} = \Theta(\log{(n)}) $$
\end{theorem}

\begin{proof}
We first show the growth rate is $\Omega(\log{(n)})$ by idetifying a value of $p$ where the bound is obtained.  Let $f$ be the function we wish to maximize:

\begin{align*}
\max_{0 < p < 1} f(p) &\geq f(\frac{1}{n}) \\
&= \log{(\frac{1}{n})} \frac{1 - (1-\frac{1}{n})^n}{n \frac{1}{n}} - \log{(\frac{1}{n})} \\
&\geq \log{(n)}[1 - 1 + (1-\frac{1}{n})^n] \\
&\geq \frac{1}{4} \log{(n)} \\
&= \Omega(\log{(n)})
\end{align*}

We now show the growth rate is $O(\log{(n)})$.  We first argue that the maximizing value $p_*$ lies within the range $\frac{1}{n} \leq p_* \leq \frac{1}{\sqrt{n}}$ as long as $n \geq 4$.  We prove that by showing the derivative of $f$ is positive for all $p \leq \frac{1}{n}$ and negative for all $p \geq \frac{1}{\sqrt{n}}$.   The derivative of $f$ is given by:

$$ \frac{d f}{d p} = \frac{1}{n p^2} \Big[1 - (1-p)^n - np - (1 - (1-p)^n - n (1-p)^{n-1} p) \log{(p)}\Big] $$

Note that the term $1 - (1-p)^n - n (1-p)^{n-1} p$ is always in the range $(0,1)$, because it can be interpreted as a probability --- namely, the it is probability that more than $1$ heads was thrown for $n$ biased coin tosses.  

Now assume $p \leq \frac{1}{n}$,

\begin{align*}
\frac{d f}{d p} &= \frac{1}{n p^2} \Big[1 - (1-p)^n - np - (1 - (1-p)^n - n (1-p)^{n-1} p) \log{(p)}\Big]  \\
&\propto 1 - (1-p)^n - np - (1 - (1-p)^n - n (1-p)^{n-1} p) \log{(p)} \\
%&\geq -(1-p)^n - (1 - (1-p)^n - n (1-p)^{n-1} p) \log{(p)} \\
&\geq 1 -(1-p)^n - np + (1 - (1-p)^n - n (1-p)^{n-1} p) \log{(n)} \\
&\geq 1 -(1-p)^n - np + (1 - (1-p)^n - n (1-p)^{n-1} p)  \\
\end{align*}

TODO...

\end{proof}

